Local-Search Based Heuristics for Advertisement Scheduling

In the MAXSPACE problem, given a set of ads A, one wants to place a subset A' of A into K slots B_1, ..., B_K of size L. Each ad A_i in A has size s_i and frequency w_i. A schedule is feasible if the total size of ads in any slot is at most L, and each ad A_i in A' appears in exactly w_i slots. The goal is to find a feasible schedule that maximizes the space occupied in all slots. We introduce MAXSPACE-RDWV, a MAXSPACE generalization with release dates, deadlines, variable frequency, and generalized profit. In MAXSPACE-RDWV each ad A_i has a release date r_i >= 1, a deadline d_i >= r_i, a profit v_i that may not be related with s_i and lower and upper bounds w^min_i and w^max_i for frequency. In this problem, an ad may only appear in a slot B_j with r_i <= j <= d_i, and the goal is to find a feasible schedule that maximizes the sum of values of scheduled ads. This paper presents some algorithms based on meta-heuristics GRASP, VNS, Local Search, and Tabu Search for MAXSPACE and MAXSPACE-RDWV. We compare our proposed algorithms with Hybrid-GA proposed by Kumar et al. (2006). We also create a version of Hybrid-GA for MAXSPACE-RDWV and compare it with our meta-heuristics. Some meta-heuristics, such as VNS and GRASP+VNS, have better results than Hybrid-GA for both problems. In our heuristics, we apply a technique that alternates between maximizing and minimizing the fullness of slots to obtain better solutions. We also applied a data structure called BIT to the neighborhood computation in MAXSPACE-RDWV and showed that this enabled ours algorithms to run more iterations.

==> conclusao.tex <==
This paper presented some variants for the MAXSPACE problem and some local-search-based heuristics for MAXSPACE and MAXSPACE-RDWV. 

We compare our algorithms with Hybrid-GA, which is the state-of-the-art in heuristics for MAXSPACE. Our best algorithms are VNS and GRASP$\plus$VNS, a GRASP version that uses VNS as a local search. Our algorithms find the best solutions among the tested algorithms in approximately~$95\%$ of instances for MAXSPACE and~$55\%$ for MAXSPACE-RDWV and guarantee an excellent solution quality for the whole set of instances. %They were not the least time-consuming, reaching the time limit of~$600$ second for more than~$80\%$ of instances for both problems. However, the algorithm previously existing in the literature Hybrid-GA also reaches the time limit in at least~$80\%$ of instances for both problems.

%In future works, %we will consider the variant in which the value of an ad is given in the input, and can be unrelated to its size. This variant is a generalization of the Multiple Knapsack Problem~\citet{chekuri2005polynomial}, which is strongly NP-hard even for $K = 2$.

